Measuring pair correlations in Bose and Fermi gases via atom-resolved microscopy

We demonstrate atom-resolved detection of itinerant bosonic $^{23}$Na and fermionic $^6$Li quantum gases, enabling the direct in situ measurement of interparticle correlations. In contrast to prior work on lattice-trapped gases, here we realize microscopy of quantum gases in the continuum. We reveal Bose-Einstein condensation with single-atom resolution, measure the enhancement of two-particle $g^{(2)}$ correlations of thermal bosons, and observe the suppression of $g^{(2)}$ for fermions; the Fermi or exchange hole. For strongly interacting Fermi gases confined to two dimensions, we directly observe non-local fermion pairs in the BEC-BCS crossover. We obtain the pairing gap, the pair size, and the short-range contact directly from the pair correlations. In situ thermometry is enabled via the fluctuation-dissipation theorem. Our technique opens the door to the atom-resolved study of strongly correlated quantum gases of bosons, fermions, and their mixtures.

==> Notes.tex <==





Points to make:

We go as close as possible to obtaining complete information about a continuous many-body system.



Requirements for this to work: System dilute enough so that resolution is not limiting.


See very clearly the different scales of pairing and interparticle spacing:
The pairing range gives the positive part of the density-density correlations, the negative stuff further out is due to the Fermi hole, given, roughly, by the interparticle spacing.

We see a repulsive molecular gas! A "Fermi hole" inherited from the fermionic nature of the constituents! This allows measuring the molecule-molecule repulsion!

Density fluctuations in the BEC-BCS crossover are a highly non-trivial subject: BCS theory gets it wrong, as Delta $N^2$ comes out non-zero. If we instead use $Delta N^2 = kappa n^2 T$, then mean-field predicts constant fluctuations at a given temperature, regardless of interaction, which is also unphysical.

Note that Delta $N^2$ gives "area law" with $V^(2/3)$ (see Zwerger)
(see PRL 1998 Giorgini, Pitaevskii und Stringari for weakly interacting BEC)



\section{References}
Important papers:
https://arxiv.org/pdf/0707.0458
[Cool: The ratio of number fluctuations between the non-interacting Fermi gas and the unitary Fermi gas should give the Bertsch]

https://journals-aps-org.libproxy.mit.edu/pra/pdf/10.1103/PhysRevA.75.063611

Castin is best:
https://arxiv.org/pdf/cond-mat/0612613

left out:

Inclusion of quantum statistical corrections close to degeneracy must go hand in hand with including the role of interparticle interactions, as otherwise unphysical results are obtained, such as an infinite density and infinite range of correlations in the homogeneous Bose gas in the limit of vanishing chemical potential. As with the equation of state~\cite{Chin, Dalibard}, understanding two-particle correlations in the interacting 2D Bose gas is a challenging problem.



